Equidistribution of currents under Anosov group actions

We study the behavior of currents on flag-manifolds under actions of Anosov subgroups of complex semisimple Lie groups G. Given a current T of bidimension (k, k) on the full flag-manifold F = G/B, we average it under the group action via a construction analogous to the construction of Patterson-Sullivan measures. We show that under certain genericity conditions (in the case of currents of integration over subvarieties), the limiting current is a Gibbs current, i.e. is given by integration (with respect to a Gibbs measure) over the flag-limit set of suitable multiples of currents of integration along Schubert varieties based at the limit points of the group. We prove that the same equidistribution result (but without any genericity assumptions) for currents defined by smooth forms on F. We also prove a form of Axiom A property for the suspension flow of the group action on F.

==> abcdefg1.tex <==


{\mini {\kap I do not think it's worth having this result as a separate corollary. We should just quote Theorem \ref{thm:thickening_distance_inequality} when needed. }



We now prove a version of Theorem \ref{thm:biholder} concerning points outside of the limit set $\La$, which is needed to understand properties of GPS currents (see Section \ref{sec_gps_currents_intersection}). 
%{\kap Recall} that a thickening $\Th\subset W$ is said to be 
 %{\em symmetric} $\Th\subset W$ if $\Th=\Th^{-1}$. For instance, every thickening of the form $\Th^k$ is symmetric. 
 

\begin{cor}\label{cor:biholder_second_version}
Suppose that $\Ga$ is an Anosov subgroup of $G$. %Zariski dense (so that every proper subvariety of $\cF$ is generic).  
Then there exists a constant $C>0$ such that the following holds for 
all $\zeta_\pm\in \geo \Ga$, thickenings $\Th\subset W$, and $x\in \Th(f(\zeta_+))$:  
%There exist positive constants $a_1,a_2,C$ and an algebraic subvariety $V\subset \cF$ (depending on $\zeta_+$ and $x$) such that for all $\zeta_-\in \geo \Ga\setminus \{\zeta_+\}$,
$$
C d_{\cF}(x, \Th(f(\zeta_-)))\geqslant  d_{\cF}(f(\zeta_-), \widehat\Th(x)). 
$$
\end{cor}
\begin{proof} Apply the theorem to $y=f(\zeta_-)$. \end{proof}


}
%The proof is similar to that of Theorem \ref{thm:biholder}. 


